Fast Eye Detector Using Siamese Network for NIR Partial Face Images

This paper proposes a fast eye detection method that is based on a Siamese network for near infrared (NIR) partial face images. NIR partial face images do not include the whole face of a subject since they are captured using iris recognition systems with the constraint of frame rate and resolution. The iris recognition systems such as the iris on the move (IOTM) system require fast and accurate eye detection as a pre-process. Our goal is to design eye detection with high speed, high discrimination performance between left and right eyes, and high positional accuracy of eye center. Our method adopts a Siamese network and coarse to fine position estimation with a fast lightweight CNN backbone. The network outputs features of images and the similarity map indicating coarse position of an eye. A regression on a portion of a feature with high similarity refines the coarse position of the eye to obtain the fine position with high accuracy. We demonstrate the effectiveness of the proposed method by comparing it with conventional methods, including SOTA, in terms of the positional accuracy, the discrimination performance, and the processing speed. Our method achieves superior performance in speed.

==> Tables/ICIPObjDetectionResults.tex <==
\begin{table}[t]
\caption{Comparison between proposed method and generic object detection methods.``Trained domain" is result for dataset with same domain as training dataset. ``Untrained domain" is result for datasets with different domain from training. ``Time" is average time taken to process input image of $96\times123$ pixels 10 times in CPU environment.}
\small
\label{tb:results2}
\begin{tabular}{llccc}
\hline
&&Proposed&YOLOv5&FRCNN\\
\hline
\begin{tabular}{l}
Trained\\
domain
\end{tabular}
&
\begin{tabular}{l}
Right\\Left
\end{tabular}
&
\begin{tabular}{l}
0.998\\0.981
\end{tabular}
&
\begin{tabular}{l}
0.983\\0.984
\end{tabular}
&
\begin{tabular}{l}
{\bf 0.999}\\{\bf 0.998}
\end{tabular}
\\ 
\begin{tabular}{l}
Untrained\\ domain
\end{tabular}
&
\begin{tabular}{l}
Right\\Left
\end{tabular}
&
\begin{tabular}{l}
{\bf 0.993}\\0.956
\end{tabular}
&
\begin{tabular}{l}
0.660\\0.608
\end{tabular}
&
\begin{tabular}{l}
0.980\\{\bf 0.982}
\end{tabular}
\\ 
\begin{tabular}{l}
Time[ms]\\
\end{tabular}
&
&
{\bf 21}&87&1970\\
\hline
\end{tabular}
\end{table}

==> abstract_en.tex <==
This paper proposes a fast eye detection method that is based on a Siamese network for near infrared (NIR) partial face images. NIR partial face images do not include the whole face of a subject since they are captured using iris recognition systems with the constraint of frame rate and resolution. The iris recognition systems such as the iris on the move (IOTM) system require fast and accurate eye detection as a pre-process. Current eye detection methods have used the results of face and its landmark detection algorithms with the assumption that the input visible light images include entire face of a subject. The eye detection performance, however, is significantly reduced when these methods are used for NIR partial face images due to the difference of data domain. Though generic object detection methods also can be used for eye detection, mostly their computational cost does not meet to the requirement of real-time iris recognition systems. Our goal is to design eye detection with high speed, high discrimination performance between left and right eyes, and high positional accuracy of eye center. Our method adopts a Siamese network and coarse to fine position estimation with a fast lightweight CNN backbone. The Siamese network improves discrimination performance by using the similarity between an input image and a single eye image prepared in advance. The network outputs features of images and the similarity map indicating coarse position of an eye. A regression on a portion of a feature with high similarity refines the coarse position of the eye to obtain the fine position with high accuracy. We demonstrate the effectiveness of the proposed method by comparing it with conventional methods, including SOTA, in terms of the positional accuracy, the discrimination performance, and the processing speed. Our method achieves superior performance in speed.
